A DPF analysis yields accurate analytic potentials for Li$_2(a\,^3\Sigma^+_u)$ and Li$_2(1\,^3 \Sigma^+_g)$ that incorporate 3-state mixing near the $1\,^3 \Sigma^+_g$-state asymptote

A combined-isotopologue direct-potential-fit (DPF) analysis of optical and photoassociation spectroscopy data for the $a\,^{3}\Sigma_u^+$ and $1\,^3\Sigma_g^+$ states of Li$_2$ has yielded accurate analytic potential energy functions for both states. The recommended M3LR$_{5,3}^{8.0}(3)$ potential for the $a\,^3\Sigma_u^+$ of $^{7,7}$Li$_2$ has a well depth of $\,{\mathfrak D}_e= 333.758(7)\,{\rm cm^{-1}}$ and equilibrium distance of $\,r_e= 4.17005(3)~$\AA, and the associated scattering lengths are $\,a_{\rm SL}= -14.759(9)\,$\AA\ for $^{7,7}$Li$_2$ and $-1906(50)\,$\AA\ for $^{6,6}$Li$_2$. For the $1\,^3\Sigma_g^+$ state, in spite of a gap of $\,\sim 5200\,{\rm cm}^{-1}$ (from $\,v(1\,^3\Sigma_g^+)= 8-61$) for which there are no data, the DPF procedure has no difficulty determining an accurate overall potential. The $1\,^3\Sigma_g^+$ state of the $^{7,7}$Li$_2$ isotopologue has a well depth of $\,{\mathfrak D}_e= 7092.417(33)\,{\rm cm^{-1}}$ and equilibrium distance of $\,r_e= 3.06524(9)~$\AA. The long-range tail of the recommended M3LR$_{6,3}^{3.6}(9)$ potential energy function for the $1\,^3\Sigma_g^+$ state is defined by the lowest eigenvalue of a $3\times 3$ long-range interstate coupling matrix to take into account the 3-state mixing near its asymptote.

==> tab_13basic.tex <==
\begin{table}[h!]
\begin{description}
\item[Table II] Dimensionless root mean square deviations $\overline{dd}$
of preliminary fits which neglected interstate coupling near the asymptote
of Li$_2(1\,^3\Sigma_g^+)$, in which the data used in the analysis was
truncated at various values of $\,v_{\rm max}\,$.
\end{description}
%
\vspace{-10mm}
\begin{center}
\[ \begin{array}{l c c c c c c c c c c}
\hline\hline
\noalign{\smallskip}
v_{\rm max} & 7 & 70 & 71 & 72 & 73 & 74 & 75 & 76 & 77 & \cdots \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\overline{dd}  & ~0.8117~ & ~0.8514~  & ~0.8975~ & ~0.9730~ & ~1.1698~ 
  & ~1.3438~ & ~1.5773~ & ~2.13601~ & ~2.8936~ & \cdots \\
%
% DRMSD  & 0.811688 & 0.851391 & 0.897455 & 0.972991 & 1.16979 & 1.34379
%        & 1.57730  & 2.13601  & 2.89365  & $\cdots$ \\
\noalign{\medskip}
\hline\hline
\end{array} \]
\end{center}
\end{table}

